Substructure of Multiquark Hadrons (Snowmass 2021 White Paper)

In recent years there has been a rapidly growing body of experimental evidence for existence of exotic, multiquark hadrons, i.e. mesons which contain additional quarks, beyond the usual quark-antiquark pair and baryons which consist of more than three quarks. In all cases with robust evidence they contain at least one heavy quark Q=c or b, the majority including two heavy quarks. Two key theoretical questions have been triggered by these discoveries: (a) how are quarks organized inside these multiquark states -- as compact objects with all quarks within one confinement volume, interacting via color forces, perhaps with an important role played by diquarks, or as deuteron-like hadronic molecules, bound by light-meson exchange? (b) what other multiquark states should we expect? The two questions are tightly intertwined. Each of the interpretations provides a natural explanation of parts of the data, but neither explains all of the data. It is quite possible that both kinds of structures appear in Nature. It may also be the case that certain states are superpositions of the compact and molecular configurations. This Whitepaper brings together contributions from many leading practitioners in the field, representing a wide spectrum of theoretical interpretations. We discuss the importance of future experimental and phenomenological work, which will lead to better understandingof multiquark phenomena in QCD.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)



==> Tcc.tex <==
%\label{sec:X(3872)}
%This LaTeX template can be useful when setting up a document to be submitted to arXiv (journal too?) as Snowmass 2021 whitepaper.

\textcolor{red} {elena writes in red}.

\textcolor{blue} {katliner writes in blue}.

 {\color{red} On the lattice there is a technical difficulty in studying exotic hadrons, such as the $X(3872)$, because their signal is buried as excitation in the short distance regime of a correlation function of the given quantum numbers. Ground states dominate Euclidean correlation functions at asymptotic times as the higher excitations are suppressed. This suppression makes it difficult to access these higher states in the spectrum. 

Motivated by this outlook, in \cite{Francis:2016hui} was preformed the search for exotic candidates that have the distinct feature of being ground states . Based on the concepts of heavy quark spin symmetry and the good diquark attractive effect,it was set the goal and performed a lattice calculation of a doubly heavy tetraquark with quantum numbers $J^P=1^+$ and flavor contents \udbb and \lsbb. It was found that both candidates exhibit significant binding below the relevant thresholds and are strong-interaction stable.

In \cite{Francis:2018jyb} this analysis was extended by varying the heavy quark mass components and it was possible to  verify that the candidates' binding energies indeed vary according to the phenomenological picture in mind, giving some tentative, yet not conclusive, evidence of its validity. In the same work it was found indication that \udcb could also be a bound state, but much shallower. The fate of this state is currently undetermined as a recent follow-up study by us did not observe signal for it any more \cite{Hudspith:2020tdf}. Additionally, in this study we performed a survey of possible candidates with different flavor combinations in addition to the quantum number channel $J^P=0^+$. We did not observe deep binding for more candidates aside of the already established \udbb and \lsbb in $J^P=1^+$. The status of shallow bound states or even resonances is not clear from this study and requires further work in the future.
 }

==> acknowledgements.tex <==
\section*{Acknowledgements}
%
%
\noindent We express our gratitude to ...



==> esposito.tex <==
\vfill\eject
\section{Key papers by Angelo Esposito}
\centerline{Institute of Physics, EPFL, 1015 Lausanne, Switzerland}
\centerline{and}
\centerline{Institute for Advanced Study, Princeton, New Jersey 08540, USA}
\centerline{\tt angeloesposito@ias.edu}
\hfill\break


In Ref.~\cite{Esposito:2021vhu}
we show that recent data on the lineshape of the $X(3872)$ point to
an effective range for the latter that is negative and  well
beyond the inverse pion mass, $r_0 \simeq -5.34$~fm. If confirmed within
experimental uncertainty, this would be a smoking gun indicating that
the $X(3872)$ is a compact tetraquark, interacting with the continuum
via standard hadronic interactions.

In Ref.~\cite{Esposito:2020ywk}
we employ the comover model to study the evolution of a tetraquark
$X(3872)$ in a hadronic medium, and compare it to the data on high
multiplicity $pp$ collisions as reported by the LHCb collaboration. We
find a behavior that nicely matches experimental data. We also use
a kinetic model to describe the evolution of meson molecules in the
same hadronic medium. We find that, while this agrees very well with
deuteron data, it fails to describe the $X(3872)$ data, hence pointing
at a compact nature of the latter.

Ref.~\cite{Esposito:2015fsa} contains
comparison between the prompt production $p_T$ spectra of the $X(3872)$
and other \emph{bona fide} molecules (deuteron, hypertriton and
helium-3). Using well tested fitted functions, we show that ALICE
and CMS data point at the fact that the production of the $X(3872)$
is at odds with a simple molecular picture. We also highlight how high
multiplicity events favor the formation of meson molecules, but disfavor
that of ordinary hadrons.


==> secwithfig.tex <==
\section{Dummy section with a figure}
\label{sec:secwithfig}

It is recommended to put figures in figs/ subdirectory to reduce a number of files in the main overleaf project directory. However, it is not necessary to specify this subdirectory in $\backslash$includegraphics directive, since it is set-up to be searched for automatically. You can then submit LaTeX source files, without modifications, with figures without dedicated subdirectory. See Fig.~\ref{fig:example} for an example. 

%\begin{figure}[tb]
\begin{figure}[b]
  \begin{center}
    \includegraphics[width=0.5\linewidth]{pentaquarks_nominal_fit_and_thresholds}
    \vspace*{-0.5cm}
  \end{center}
  \caption{
    \small 
        Distribution of $\jpsi p$ mass in 
        $\Lb\to\jpsi p \Kp$ decays fit with 3 $P_c^+$ states and polynomial background from Ref.~\cite{LHCb:2019kea}.}
  \label{fig:example}
\end{figure}

\clearpage   % to force the figure to be placed beforre the following text
